Asymptotic analysis of a Neumann problem in a domain with cusp. Application to the collision problem of rigid bodies in a perfect fluid

We study a two dimensional collision problem for a rigid solid immersed in a cavity filled with a perfect fluid. We are led to investigate the asymptotic behavior of the Dirichlet energy associated to the solution of a Laplace Neumann problem as the distance $\varepsilon>0$ between the solid and the cavity's bottom tends to zero. Denoting by $\alpha>0$ the tangency exponent at the contact point, we prove that the solid always reaches the cavity in finite time, but with a non zero velocity for $\alpha <2$ (real shock case), and with null velocity for $\alpha \geqslant 2$ (smooth landing case). Our proof is based on a suitable change of variables sending to infinity the cusp singularity at the contact. More precisely, for every $\varepsilon\geqslant 0$, we transform the Laplace Neumann problem into a generalized Neumann problem set on a domain containing a horizontal strip $]0,\ell_\varepsilon[\times ]0,1[$, where $\ell_\varepsilon\to +\infty$.

==> change_of_variables.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'change_of_variables.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{220.15483398bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.63939902)%
    \put(0,0){\includegraphics[width=\unitlength]{change_of_variables.pdf}}%
    \put(0.20980621,0.2743478){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.47849838,0.27434795){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$0$}}}%
    \put(0.04901899,0.40860532){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Omega_\varepsilon\setminus\overline{\mathcal V}_\varepsilon$}}}%
    \put(0.2221555,0.54497603){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon$}}}%
    \put(0.56798828,0.3433418){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon$}}}%
    \put(0.29569944,0.3498895){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal V_\varepsilon$}}}%
    \put(0.29569941,0.43679522){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma_\varepsilon$}}}%
    \put(0.20980621,0.00470981){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.29783134,0.1188943){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$R_\varepsilon$}}}%
    \put(0.29569943,0.21620683){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma_\varepsilon$}}}%
    \put(0.87087253,0.00470969){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\ell_\varepsilon$}}}%
    \put(0.01754393,0.1188945){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$D=\omega_\varepsilon\setminus \overline{R}_\varepsilon$}}}%
    \put(0.47849838,0.0047097){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$0$}}}%
    \put(0.95254094,0.10858025){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{1}}}%
  \end{picture}%
\endgroup%


==> dessin5.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dessin5.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{249.22658691bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.67251064)%
    \put(0,0){\includegraphics[width=\unitlength]{dessin5_hal.pdf}}%
    \put(0.36068719,0.01955256){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$0$}}}%
    \put(0.44073502,0.10370482){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon$}}}%
    \put(0.16932455,0.01955256){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta'$}}}%
    \put(0.30080291,0.11670801){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_1$}}}%
    \put(0.24221557,0.45457665){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_2$}}}%
    \put(0.08625174,0.55958104){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_3$}}}%
    \put(0.2176048,0.01955255){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.94214313,0.0201806){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$0$}}}%
    \put(0.74436063,0.0201806){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta'$}}}%
    \put(0.88225885,0.11733605){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_1$}}}%
    \put(0.82367151,0.45520469){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_2$}}}%
    \put(0.66770768,0.56020908){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$U_3$}}}%
    \put(0.79906074,0.02018059){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.08586639,0.01955256){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta''$}}}%
    \put(0.66365337,0.01955256){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta''$}}}%
  \end{picture}%
\endgroup%


==> dessin_6.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dessin_6.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{181.1203125bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.51728567)%
    \put(0,0){\includegraphics[width=\unitlength]{dessin_6_hal.pdf}}%
    \put(0.13252588,-0.00104383){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{0}}}%
    \put(0.53446864,-0.00104383){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta$}}}%
    \put(0.83482148,-0.00104383){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta'$}}}%
    \put(-0.07933018,0.3116134){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$H(\zeta)+\varepsilon$}}}%
    \put(0.10726885,0.26280875){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon$}}}%
    \put(0.26501723,0.15459339){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O_1$}}}%
    \put(0.59628874,0.15459339){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O_2$}}}%
    \put(0.75088211,0.26501723){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O_3$}}}%
  \end{picture}%
\endgroup%


==> dessin_fourth.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dessin_fourth.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{265.3375bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.53571246)%
    \put(0,0){\includegraphics[width=\unitlength]{dessin_fourth_hal.pdf}}%
    \put(0.38966077,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{0}}}%
    \put(0.59887846,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta$}}}%
    \put(0.67379481,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta'$}}}%
    \put(0.74871132,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta''$}}}%
    \put(0.17514019,0.07382846){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$-\zeta$}}}%
    \put(0.08629599,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$-\zeta'$}}}%
    \put(-0.00254813,0.07382846){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$-\zeta''$}}}%
    \put(0.54270501,0.35175976){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O$}}}%
    \put(0.04069085,0.49244973){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon$}}}%
    \put(0.04069085,0.27891651){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon^{++}$}}}%
    \put(0.04069085,0.3858803){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon^+$}}}%
    \put(0.60300557,0.39698522){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O^+$}}}%
    \put(0.6783813,0.42713548){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O^{++}$}}}%
  \end{picture}%
\endgroup%


==> dessin_fourth_bis.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dessin_fourth_bis.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{265.3375bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.53571246)%
    \put(0,0){\includegraphics[width=\unitlength]{dessin_fourth_bis_hal.pdf}}%
    \put(0.39569083,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{0}}}%
    \put(0.59887846,0.07382856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta$}}}%
    \put(0.17514019,0.07382846){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$-\zeta$}}}%
    \put(0.42210396,0.38290856){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O$}}}%
    \put(0.04069085,0.49244973){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon$}}}%
    \put(0.04069085,0.27891651){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon^{++}$}}}%
    \put(0.04069085,0.3858803){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon^+$}}}%
    \put(0.42210396,0.4733594){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O^{++}$}}}%
    \put(0.42210396,0.42813397){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O^{+}$}}}%
  \end{picture}%
\endgroup%


==> dessin_fourth_ter.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'dessin_fourth_ter.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{154.94459229bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.75583399)%
    \put(0,0){\includegraphics[width=\unitlength]{dessin_fourth_ter_hal.pdf}}%
    \put(0.47657438,0.10899039){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{0}}}%
    \put(0.71144455,0.10899039){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\zeta$}}}%
    \put(0.2417042,0.10899039){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$-\zeta$}}}%
    \put(0.54212922,0.46984537){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O$}}}%
    \put(0.05947745,0.64539204){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon$}}}%
    \put(0.54212922,0.59892374){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal O^{+}$}}}%
    \put(0.05947741,0.38676235){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Omega_\varepsilon$}}}%
  \end{picture}%
\endgroup%


==> graphe_rho_new.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'graphe_rho_new.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{399.58623047bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.45604563)%
    \put(0,0){\includegraphics[width=\unitlength]{graphe_rho_new_hal.pdf}}%
    \put(0.42555609,0.40612799){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\ell_\varepsilon$}}}%
    \put(0.42555606,0.44202781){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1$}}}%
    \put(0.44836515,0.22547727){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\xi_1$}}}%
    \put(0.27532005,0.22547728){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.22623256,0.22547728){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^-$}}}%
    \put(0.34306517,0.22547727){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^+$}}}%
    \put(-0.00052837,0.0771523){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1=\frac{1}{1+\varepsilon}\xi_1+\frac{\delta\varepsilon}{1+\varepsilon}$}}}%
    \put(0.21151452,0.02389512){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1=\xi_1$}}}%
    \put(0.42435533,0.09158446){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.42435538,0.13396015){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$s_\varepsilon$}}}%
    \put(0.42435534,0.04991632){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^-$}}}%
    \put(0.84999512,0.44202781){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1$}}}%
    \put(0.87280418,0.22547727){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\xi_1$}}}%
    \put(0.6997591,0.22547728){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.65067165,0.22547728){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^-$}}}%
    \put(0.76750422,0.22547727){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^+$}}}%
    \put(0.6359536,0.02389512){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$x_1=\xi_1$}}}%
    \put(0.84879439,0.09158447){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.84879443,0.16198917){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$s_{\varepsilon=0}$}}}%
    \put(0.84879439,0.04991632){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta^-$}}}%
    \put(0.15945066,0.4089945){\color[rgb]{0.61568627,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon>0$}}}%
    \put(0.591326,0.4089945){\color[rgb]{0.61568627,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon=0$}}}%
  \end{picture}%
\endgroup%


==> miscellanious.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'miscellanious.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{290.56369629bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.86571227)%
    \put(0,0){\includegraphics[width=\unitlength]{miscellanious_hal.pdf}}%
    \put(0.04926474,0.77005837){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Omega_\varepsilon$}}}%
    \put(0.34828141,0.47218249){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon$}}}%
    \put(0.0495947,0.59014672){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma_\varepsilon$}}}%
    \put(0.12975936,0.6871407){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_\varepsilon$}}}%
    \put(0.55005032,0.77005837){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Omega_0$}}}%
    \put(0.55992652,0.51898807){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma_0$}}}%
    \put(0.64531285,0.64387112){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$S_0$}}}%
    \put(0.46501903,0.16077678){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$D$}}}%
    \put(0.69798467,0.10679698){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$R_\varepsilon^r$}}}%
    \put(0.09710356,0.10679698){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$R_\varepsilon^l$}}}%
    \put(0.06760146,0.47878232){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal V_\varepsilon^l$}}}%
    \put(0.13633503,0.46319525){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\mathcal V_\varepsilon^r$}}}%
  \end{picture}%
\endgroup%


==> simple_case.tex <==
%% Creator: Inkscape inkscape 0.48.2, www.inkscape.org
%% PDF/EPS/PS + LaTeX output extension by Johan Engelen, 2010
%% Accompanies image file 'simple_case.pdf' (pdf, eps, ps)
%%
%% To include the image in your LaTeX document, write
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics{<filename>.pdf}
%% To scale the image, write
%%   \def\svgwidth{<desired width>}
%%   \input{<filename>.pdf_tex}
%%  instead of
%%   \includegraphics[width=<desired width>]{<filename>.pdf}
%%
%% Images with a different path to the parent latex file can
%% be accessed with the `import' package (which may need to be
%% installed) using
%%   \usepackage{import}
%% in the preamble, and then including the image with
%%   \import{<path to file>}{<filename>.pdf_tex}
%% Alternatively, one can specify
%%   \graphicspath{{<path to file>/}}
%% 
%% For more information, please see info/svg-inkscape on CTAN:
%%   http://tug.ctan.org/tex-archive/info/svg-inkscape
%%
\begingroup%
  \makeatletter%
  \providecommand\color[2][]{%
    \errmessage{(Inkscape) Color is used for the text in Inkscape, but the package 'color.sty' is not loaded}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\transparent[1]{%
    \errmessage{(Inkscape) Transparency is used (non-zero) for the text in Inkscape, but the package 'transparent.sty' is not loaded}%
    \renewcommand\transparent[1]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \ifx\svgwidth\undefined%
    \setlength{\unitlength}{407.04221191bp}%
    \ifx\svgscale\undefined%
      \relax%
    \else%
      \setlength{\unitlength}{\unitlength * \real{\svgscale}}%
    \fi%
  \else%
    \setlength{\unitlength}{\svgwidth}%
  \fi%
  \global\let\svgwidth\undefined%
  \global\let\svgscale\undefined%
  \makeatother%
  \begin{picture}(1,0.46417392)%
    \put(0,0){\includegraphics[width=\unitlength]{simple_case_hal.pdf}}%
    \put(0.15551528,0.34552938){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma^i_\varepsilon$}}}%
    \put(0.14577422,0.18211411){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma^e$}}}%
    \put(0.44058393,0.24697222){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma^b_\varepsilon$}}}%
    \put(0.00623094,0.29610718){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Gamma^t_\varepsilon$}}}%
    \put(0.08844291,0.27089099){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\Omega_\varepsilon$}}}%
    \put(0.35214099,0.14280613){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma^i_\varepsilon$}}}%
    \put(0.00623095,0.0700864){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma^t$}}}%
    \put(0.69378558,0.07631656){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma^b_\varepsilon$}}}%
    \put(0.25550174,0.00556223){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\gamma^e_\varepsilon$}}}%
    \put(0.21619378,0.07861592){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\omega_\varepsilon$}}}%
    \put(0.50538808,0.24076127){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\varepsilon$}}}%
    \put(0.03958874,0.18211409){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.03958874,0.00556223){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta$}}}%
    \put(0.42466639,0.18211409){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$0$}}}%
    \put(0.3063915,0.18211409){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\delta'$}}}%
    \put(0.49380626,0.00556223){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\ell_\varepsilon'$}}}%
    \put(0.67560565,0.00556223){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{$\ell_\varepsilon$}}}%
    \put(0.7521157,0.07300049){\color[rgb]{0,0,0}\makebox(0,0)[lb]{\smash{1}}}%
  \end{picture}%
\endgroup%

